Parallel Shortest-Paths Using Radius Stepping

The single-source shortest path problem (SSSP) with nonnegative edge weights is a notoriously difficult problem to solve efficiently in parallel---it is one of the graph problems said to suffer from the transitive-closure bottleneck. In practice, the $\Delta$-stepping algorithm of Meyer and Sanders (J. Algorithms, 2003) often works efficiently but has no known theoretical bounds on general graphs. The algorithm takes a sequence of steps, each increasing the radius by a user-specified value $\Delta$. Each step settles the vertices in its annulus but can take $\Theta(n)$ substeps, each requiring $\Theta(m)$ work ($n$ vertices and $m$ edges). In this paper, we describe Radius-Stepping, an algorithm with the best-known tradeoff between work and depth bounds for SSSP with nearly-linear ($\otilde(m)$) work. The algorithm is a $\Delta$-stepping-like algorithm but uses a variable instead of fixed-size increase in radii, allowing us to prove a bound on the number of steps. In particular, by using what we define as a vertex $k$-radius, each step takes at most $k+2$ substeps. Furthermore, we define a $(k, \rho)$-graph property and show that if an undirected graph has this property, then the number of steps can be bounded by $O(\frac{n}{\rho} \log \rho L)$, for a total of $O(\frac{kn}{\rho} \log \rho L)$ substeps, each parallel. We describe how to preprocess a graph to have this property. Altogether, Radius-Stepping takes $O((m+n\log n)\log \frac{n}{\rho})$ work and $O(\frac{n}{\rho}\log n \log (\rho{}L))$ depth per source after preprocessing. The preprocessing step can be done in $O(m\log n + n\rho^2)$ work and $O(\rho^2)$ depth or in $O(m\log n + n\rho^2\log n)$ work and $O(\rho\log \rho)$ depth, and adds no more than $O(n\rho)$ edges.

==> complexity-save.tex <==
Now we analyze the work and depth for the \AlgName{} algorithm.
%Here we assume that $N^*(\cdot)$, the $\rho$-nearest-neighbor sets for all vertices, are explicitly computed using Dijkstra's algorithm, as well as the the distance to the vertices in the sets.  This is legitimate from a theoretical point of view, although in practice this might require too much storage space, and we will show how to handle this problem in the next section.
Thorough the complexity analysis we assume $B(v,r(v))\ge \rho$ for all $v\in V$, and we show how to pre-process the graph to guarantee this property in the next section.
The pseudocode of an efficient implementation is shown in Algorithm~\ref{alg:efficientversion}, which is used as a \yan{don't know whether ``reference'' is the correct word here} for the analysis.

There are essentially two steps in Algorithm~\ref{alg:sssp} that are costly and require efficient solutions: to calculate the round distance $d_i$ (line~\ref{line:computeleadnode}); to find all unvisited vertices with tentative distances less than $d_i$ (line~\ref{line:innerloop}).

To efficiently support these two queries, we use two ordered sets $Q$ and $R$ implemented by balanced binary search trees to store the tentative distance ($\delta(u)$) for each unvisited node and the tentative distance plus the vertex radius ($\delta(u)+r(u)$).   With these two BSTs, the selection of round distance corresponds to get the minimum element in the tree $R$, and picking vertices within a certain distance is a split operation of the BST $Q$.  Both operations require $O(\log n)$ work.

Let $A_i$ be the \defn{active set} that contains the elements visited in the $i$-th round (all $u$ in line~\ref{line:innerloop} in Algorithm~\ref{alg:sssp}) and computed by splitting the BST $Q$ in line~\ref{line:split} in Algorithm~\ref{alg:efficientversion}.   To maintain the priority queues sequentially, we relax all neighbors of vertices in $A_i$ for $k+2$ substeps.  Other than update the tentative distance, the status of the neighbor vertex (refer as $v$) may have three conditions: (1) if the previous distance of $v$ is already no more than $d_i$, $v$ is already removed from $Q$ and $R$ in earlier this step so we do nothing; (2) if the previous distance is larger than $d_i$ while the updated value is no more than $d_i$, we remove $v$ from $Q$ and $R$, and add $v$ to the active set $A_i$; (3) if the updated distance is still larger than $d_i$, we decrease the keys corresponding to $v$ in $Q$ and $R$.

\begin{lemma}[correctness]
The efficient version with BSTs $Q$ and $R$ (Algorithm~\ref{alg:efficientversion}) visits the same vertices in each step comparing to Algorithm~\ref{alg:sssp}, and computes the shortest-path distances correctly.
\end{lemma}

For the compactness of the analysis of work and depth, the proof is given in appendix.

The key step to parallelize Algorithm~\ref{alg:efficientversion} is to handle the inner loop (line~\ref{line:innerloop2}), which can be partitioned into two parts: to update the tentative distances, and to update the BSTs.  We process these two step one after the other.  To update the tentative distances, we just use priority-write (\mf{WriteMin}) to relax the other endpoints for all edges that have endpoints in $A_i$.  After all tentative distances are updated, each edge checks whether the relaxation (priority-write) is successful or not.  If succeeded, the edge will \emph{own} this vertex, and create a node that contains the vertex label (second key) \yan{is this the correct English word?} and current tentative distance (first key).  Then we create a BST that contains all these nodes using standard parallel packing and sorting process.  With this BST, we first apply \mf{difference} operation to remove out-of-date keys in $Q$, then we \mf{split} this BST into two parts by $d_i$, and \mf{union} each part separately with $A_i$ and $Q$.  It is easy to see that in this parallel version we apply asymptotically the same number operations to $Q$ comparing to the sequential version.  We can maintain $R$ in a similar way.

Now let's analyze the work and depth of the parallel version.  Each vertex is only in the active set in one round, so each of its neighbors is relaxed $k+2$ times, once in each substep.  In the worst case that all the relaxation succeeded, there are $O(m)$ updates for $Q$ and $R$, each can be done for no more than $O(k)$ times.  Assume the number of updates in round $i$ is $a_i$, then we have $\sum_i{a_i}=m$.  The work and depth for set \mf{difference} and \mf{union} are $O(p\log (q/p))$ and $O(\log p\log q)$ for two sets with size $p$ and $q(>p)$.  The overall work $W$ for all set operations is no more than $\sum_i{a_i\cdot k\log n}=mk\log n$, and the depth $D$ is no larger than $O(\sum_i{k\log a_i\log n})=O(k\log n\sum_i{\log a_i})$.  Due to the concavity of the logarithm function, we have:
\begin{align*}
D&= O\left(k\log n\sum_i{\log a_i}\right)\\
&= O\left(k\log n \cdot {n\over \rho}\log \rho L\cdot{\log {m\over (n/\rho)\log \rho L}}\right)\\
&= O\left(k{n\over \rho}\log n \log{\rho m\over n} \log\rho L\right)
\end{align*}
%when $\rho\ge m/n$, and an extra $\log(m/n)$ term otherwise.
All other steps in Algorithm~\ref{alg:efficientversion} are inexpensive comparing to the cost to maintain the BSTs.
Since we can set $k$ to be any positive integer in the preprocessing, we can assume $k=1$ (larger $k$ only for implementation purpose), and
this leads the following lemma:

\begin{lemma}
The \AlgName{} algorithm computes single-source shortest-path in $O(m)$ work and $O\left((n/\rho)\log n \log{\rho m\over n} \log\rho L\right)$ depth.
\end{lemma}

\begin{algorithm}[t]
\caption{The Shortest-path Algorithm.}
\label{alg:efficientversion}
\KwIn{A graph $G=(V,E,w)$, vertex radii $r(\cdot)$ and a source node $s$.}
\KwOut{The graph distances $\delta(\cdot)$ from $s$.}
    \vspace{0.5em}
%$S_0\leftarrow \{s\}$\\
\DontPrintSemicolon
$\delta(\cdot)\leftarrow +\infty$, $\delta(s)\leftarrow 0$\\
$i\leftarrow 1$\\
$Q=\{w(s,u)\,|\,u\in N(s)\}$\\
$R=\{w(s,u)+r(u)\,|\,u\in N(s)\}$\\
\While{$|Q|>0$\label{line:loop}} {
$d_{i}\leftarrow R.\mf{extract-min}()$\\
$\{A_i,Q\}=Q.\mf{split}(d_i)$\label{line:split}\\
\lForEach {$u\in A_i$} {$R.\mf{remove}(u)$}
%\For{$k'\leftarrow 1$ to $k$} {
%\ForEach{$u\in A_i, v\in N(u)$} {
%\ForEach{$u\in A_i, v\in N^*(u)$\label{line:innerloop1}} {
%    \mf{update}($u$, $v$, $w^*(u,v)$)
%}
\Repeat{no $\delta(v)$ that $v\in A_i$ is updated\label{line:substeploop}} {
    \ForEach{$u\in A_i, v\in N(u)$\label{line:innerloop2}} {
    %    \mf{update}($u$, $v$, $w(u,v)$)
    \If {$\delta(v)>\delta(u)+w(u,v)$} {
    \If {$\delta(v)>d_i$ \emph{and} $\delta(u)+w(u,v)\le d_i$} {
    $R.\mf{remove}(v)$\\
    $Q.\mf{remove}(v)$\\
    $A_i.\mf{insert}(v)$
    }
    $\delta(v)=\delta(u)+w(u,v)$\\
    \If {$\delta(v)>d_i$} {
    $Q.\mf{decrease-key}(v,\delta(v))$\\
    $R.\mf{decrease-key}(v,\delta(v)+r(v))$
    }
    }
}
}
%}
%$S_i=S_{i-1}+A_i$\\
$i=i+1$\\
}
\Return {$\delta(\cdot)$}\\[.25em]

\hide{
  \SetAlgoLined
  \SetKwFunction{algo}{algo}\SetKwFunction{funcName}{update}
  \SetKwProg{myfunc}{function}{}{}
  \myfunc{\mf{update}\emph{(vertex $u$ and $v$, distance $w$)}}{
\If {$\delta(v)>\delta(u)+w$} {
\If {$\delta(v)>d_i$ \emph{and} $\delta(u)+w\le d_i$} {
$R.\mf{remove}(v)$\\
$Q.\mf{remove}(v)$\\
$A_i.\mf{insert}(v)$
}
$\delta(v)=\delta(u)+w$\\
\If {$\delta(v)>d_i$} {
$Q.\mf{decrease-key}(v,\delta(v))$\\
$R.\mf{decrease-key}(v,\delta(v)+r(v))$
}
}
  }
  }
\end{algorithm}  

==> correctness.tex <==
The proof for correctness shows that for each vertex $v\in V$, if its distance to the source node is less than the $i$-th step distance, this $\delta(v)$ is correctly computed to be $d(s,v)$ after the $i$-th step.

\begin{lemma}\label{lem:correctness}
For given vertex radii $r(\cdot)\le\bar{r}_k(\cdot)$, for all $v\in V$, if $d(s,v)<d_i$, then at the end of the $i$-th step, we have $\delta(v)=d(s,v)$, which further leads to $v\in S_i$.
\end{lemma}

\begin{proof}
We prove by induction that in the $i$-th round, all vertices with distances less than $d_{i-1}$ are properly computed and all of their outgoing edges are relaxed.  Clearly the base case holds for the source node with distance 0 (line~\ref{line:init1} to~\ref{line:init2}).

We now look at vertex $v$ s.t. $d_{i-1}\le d(s,v)< d_i$.  Consider the shortest path from $s$ to $v$ and let $u$ be the first node on the path that is not in $S_{i-1}$.  Based on the induction, we have $\delta(u)=d(s,u)$ at the beginning of this step.
Also, the step distance $d_i\le \delta(u)+r(u)\le\delta(u)+\bar{r}_k(u)$ must be satisfied after line~\ref{line:computeleadnode}.
Notice that $v$ is no more than $k$-hop away from $u$, since otherwise $d(s,v)=\delta(u)+d(u,v)\ge\delta(u)+\bar{r}_k(u)\ge \delta(u)+r(u)\ge d_i$.
This means that $\delta(v)$ is correctly computed in the first $k$ substeps, and $v$'s neighbors are relaxed in the $(k+1)$-th substeps.
%Since $u$ is on the shortest path to $v$, we have $d(u,v)< d_i-\delta(u)\le r(u)$, so that $v$ is in $N^*(u)$.  This shows that $\delta(v)$ is updated in line~\ref{line:updatealldelta} to its final value, and $v$ is added to $S_i$ later in line~\ref{line:updateneighbor}.
\end{proof}

Based on Lemma~\ref{lem:correctness}, the distance from the source node to each vertex is correctly computed, and this gives the correctness of the \AlgName{} Algorithm. 

==> proof.tex <==
\section{Temp: Proof for Correctness}
After each round the $\delta(\cdot)$ for each node $v$ in $S_i$ will never be update in the future round, meaning that the shortest distance calculation is done for any $v\in S_i$. We need to prove that when a vertex is added into $S_i$, the current $\delta(\cdot)$ is exact the shortest distance from the source.
\begin{lemma}
\label{lem:correctness1}
After round $i$ in \AlgName{} if $\delta(v)\le d_i$, then $\delta(v)=d(s,v)$.
\end{lemma}
\begin{proof}
Assume to the contrary that $\delta(v)\ge d(s,v)$. Suppose on the shortest path from $s$ to $v$ there is an edge $e=(x,y)$ where $x\in S_{j-1}$ and $y\notin S_{j-1}$. According to our hypothesis, $y\ne v$. Also, since $(x,y)$ is on the shortest path from $s$ to $v$, the path from $s$ to $y$ via $x$ is also the shortest path from $s$ to $y$, which means at this point $\delta(y)=d(s,y)\le d(s,v)\le d_i$. Since in Line \ref{line:updatealldelta} we update any $v'\in N^*(y)\backslash S_{i-1}$ that $\delta(v')\leftarrow \min\{\delta(v'), \delta(y)+w^*(y,v')\}$, the only possibility that $\delta(v)$ has not been updated to $d(s,v)$ is that $v$ is not in $y$'s \ourstructure{k}{\rho}. Thus $d(v,y)>r(y)$. We have:
\begin{align*}
d_i &\le \delta(y)+r(y) <\delta(y)+d(v,y)=d(s,y)+d(y,v)\\
&=d(s,v) \le \delta(v)
\end{align*}
This violates our hypothesis that $\delta(v)\le d_i$.
\end{proof}

Also, we need to show that after round $i$, all vertices within distance $d_i$ to source will be visited and be added to $S_i$.
\begin{lemma}
\label{lem:correctness2}
After round $i$ in \AlgName{} if $d(s,v)\le d_i$, then $v$ will be added to $S_i$.
\end{lemma}
\begin{proof}
Assume to the contrary that there exists some $v\in V\backslash S{i}$ who satisfies $d(s,v)\le d_i$. Suppose on the shortest path from $s$ to $v$ there is an edge $e=(x,y)$ where $x\in S_{j-1}$ and $y\notin S_{j-1}$. According to our hypothesis, $y\ne v$. Also, since $(x,y)$ is on the shortest path from $s$ to $v$, the path from $s$ to $y$ via $x$ is also the shortest path from $s$ to $y$, which means at this point $\delta(y)=d(s,y)$. Since in Line \ref{line:updatealldelta} we update any $v'\in N^*(y)\backslash S_{i-1}$ that $\delta(v')\leftarrow \min\{\delta(v'), \delta(y)+w^*(y,v')\}$, the only possibility that $\delta(v)$ has not been updated to $d(s,v)$ is that $v$ is not in $y$'s \ourstructure{k}{\rho}. Then for the same reason as the proof of Lemma \ref{lem:correctness1} we can get $d_i<d(s,v)$, leading to a contradiction.
\end{proof}


\section{TEMP: Proof for Number of Rounds}
In \AlgName{}, it is clear to see that $S_j-S_i$ is the set of nodes visited in round from $i+1$ to $j$. Recall that the \emph{lead node} $v$ in round $i$ is an unvisited node that $\delta(v)+r(v)=d_i$.

We claim the following theorem:
\begin{theorem}
\label{thm:round}
In any $t>\log \rho L$ consecutive rounds, either we have finished visiting all the nodes in $V$, or $|S_{i+t}-S_i|\ge \rho$.
\end{theorem}

Our analysis starting from round $i$ and ending with some $j>i$. We call the status at round $i$ the \emph{context}. We show that if $|S_{j+1}-S_{i}|$ is less than $\rho$, the difference in round distance, which is $d_j-d_i$ will double in round $j$, i.e., $d_j-d_i>2(d_{j-1}-d_i)$.

We first prove some lemmas.

\begin{lemma}
\label{lem:outnodes}
If $v\in V\backslash S_i$, we have $d(s,v)>d_i$.
\end{lemma}
This lemma is equivalent to Lemma \ref{lem:correctness2}.

\begin{lemma}
%\label{lem:deltaleadnode}
%In round $j$ in the algorithm \AlgName{}, there exist a lead node $v$ in this round, which satisfies $\delta(v)=d(s,v)$ after Line \ref{line:updateneighbor}.
In round $j$ in the algorithm \AlgName{}, the lead node $v$ in this round satisfies $\delta(v)=d(s,v)$ after Line \ref{line:updateneighbor}.
\end{lemma}
\begin{proof}
Assume to the contrary that $\delta(v)>d(s,v)$, meaning that the shortest path is more than one hop from $S_{j-1}$ to $v$. Suppose on the shortest path from $s$ to $v$ there is an edge $e=(x,y)$ where $x\in S_{j-1}$ and $y\notin S_{j-1}$. According to our hypothesis, $y\ne v$. Also, since $(x,y)$ is on the shortest path from $s$ to $v$, the path from $s$ to $y$ via $x$ is also the shortest path from $s$ to $y$, which means at this point $\delta(y)=d(s,y)$.

%If $r(y)\le d(y,v)$, then $\delta(y)+r(y)\le d(s,y)+r(y)\le d(s,y)+d(y,v)=d(s,v)\le \delta(v)\le \delta(v)+r(v)$, which violate that $v$ is the lead node. Thus we must have $r(y)>d(y,v)$, which means that $v\in N^*(y)$.
If $r(y)< d(y,v)+r(v)$, then $\delta(y)+r(y)< \delta(y)+d(y,v)+r(v)\le \delta(v)+r(v)$, which violates that $v$ is the lead node.

Thus $r(y) \ge d(y,v)+r(v)$. In this case for any $v'\in N^*(v)$, $d(y,v')\le d(y,v)+d(v,v')\le d(y,v)+r(v)\le r(y)$, meaning that $N^*(v)\subseteq N^*(y)$. Since $|N^*(v)|=|N^*(y)|=\rho$, we have $N^*(v)=N^*(y)$. Denote the set as $N^*$, for any $v'\in N^*$, $d(y,v')\le d(y,v)+d(v,v')\le d(y,v)+r(v)$. Notice that $r(y)=\max_{v'\in N^*}d(y,v')$, we must have $r(y)\le d(y,v)+r(v)$. Combining with $r(y) \ge d(y,v)+r(v)$ it leads to $r(y) = d(y,v)+r(v)$. Therefore $\delta(y)+r(y)=\delta(y)+d(y,v)+r(v)=d(s,v)+r(v)\le \delta(v)+r(v)$, leading to a contradiction to the assumption that $v$ is the lead node.
\end{proof}
%Notice that there could be multiple lead nodes in a round, but at least one of them satisfies $\delta(\cdot)$ is the exact distance from the source. In the following proof, when we talk about ``lead nodes'' it especially refers to those with $\delta(v)=d(s,v)$.

Now we show that if $v$ is a lead node of round $j$, and the radius of $v$ is less than the distance from $v$ to the context, then all the nodes in $v$'s nearby list should appear in $S_{j}-S_i$.

\begin{lemma}
\label{lem:neighbor}
If $v$ is the lead node in round $j$ ($j>i$) where $\delta(v)+r(v)=d_j$, if $r(v)<d(s,v)-d_i$, we have $N^{*}(v)\subseteq (S_{j}-S_{i})$.
\end{lemma}
\begin{proof}
For each $v'\in l[v]$ we prove that $v'$ should also in $S_{j}-S_i$.

If $v'\in N^*(v)$, we have $d(v,v')\le r(v)$. This indicates $d(s,v')\le d(s,v)+d(v,v')\le \delta(v)+r(v)=d_j$. According to Lemma \ref{lem:correctness2}, $v'$ must be included by $S_j$. Now we prove that $v'$ cannot appear in $S_{i}$.

Notice $d(v',v)\le r(v) <d(s,v)-d_i$. If $v'$ is in $S_{i}$, we should have $d(v',v)\ge d(s,v)-d_i$. This leads to a contradiction.

To sum up, $\forall v'\in N^*(v)$, $v'$ must be in $S_{j}$, but not in $S_i$.
\end{proof}


Now we show that at round $j$, either we have explored $\rho$ nodes, or the context distance should double.
\begin{lemma}
%\label{lem:double}
%$\forall j>i$, either $|S_j-S_i| \ge \rho$, or $D_m(j+1)\ge 2D_m(j)$.
$\forall j>i$, either $|S_{j}-S_i| \ge \rho$, or $d_j-d_i>2(d_{j-1}-d_i)$.
\end{lemma}
\begin{proof}
For the lead node $v$ where where $\delta(v)+r(v)=d_j$, from Lemma \ref{lem:neighbor}, either $r(v)\ge d(s,v)-d_i$, or $r(v)<d(s,v)-d_i$ which leads to $N^*(v)\subseteq S_{j+1}-S_i$. The later one indicates $|S_{j}-S_i| \ge |N*(v)|=\rho$.

If $r(v)\ge d(s,v)-d_i$, then in the next step, we will extend at least the length of $d(s,v)-d_i$ further from the context $F_i$. Also, since $v\notin S_{j-1}$, according to Lemma \ref{lem:outnodes}, we have $d(s,v)>d_{j-1}$. Notice that for lead node $v$, $\delta(v)=d(s,v)$ (Lemma \ref{lem:deltaleadnode}).
\begin{align*}
d_j-d_i&=\delta(v)+r(v)-d_i \\
&\ge d(s,v)+\left(d(s,v)-d_i\right)-d_i\\
&=2(d(s,v)-d_i)>2(d_{j-1}-d_i)
\end{align*}
\end{proof}

\begin{lemma}
\label{lem:distance}
$\forall j>i$, either $|S_{j+1}-S_i| \ge \rho$, or $d_j-d_i>2^{j-i}$.
\end{lemma}
This directly follows Lemma \ref{lem:double} since after normalizing the minimum edge weight is $1$.

Now we show the proof for Theorem \ref{thm:round}
\begin{proof} [\textbf{Theorem \ref{thm:round}}]
Assume $t=\log \rho L$. According to Lemma \ref{lem:distance} either $|S_{i+t'}-S_i| \ge \rho$, or we have $d_{i+t}-d_{i}>2^{t}=\rho L$. This means either we have finished visiting all the nodes, or any unvisited node $u$ should have $d(s,u)>d_{i+t}>d_{i}+2^{t}$. Specially, for $u^*=\arg\min d(s,u^*)-d_i$, we have $d(s,u^*)-d_i>\rho L$. Suppose $v^*=\arg\min_{v\in S_i} d(v,u^*)$. All the nodes on the path from $u^*$ to $v^*$ should appear in $S_{j}-S_{i}$ (otherwise it violates the definition of $u^*$ or $v^*$), and the path is at least of length $\rho L$. Considering that $L$ is the heaviest edge weight, there should be at least $\rho$ vertices on the path. In that case, we still have $|S_j-S_i|\ge \rho$. In summary, in $t=t'+1=\log \rho L+1$ rounds, we have $|S_{i+t}-S_i|\ge \rho$.
\end{proof}

Theorem \ref{thm:numberofrounds} directly follows Theorem \ref{thm:round}. 
